Bidirectional Wireless Communication for Weakly Coupled Implantable Brain-Computer Interfaces

Implantable brain-computer interfaces (BCIs) promise transformative societal impact, from restoring lost motor, sensory, and speech function in patients with paralysis, stroke, sclerosis, and sensory deficits to serving as a high-bandwidth conduit between human cognition and machine intelligence. Realizing these visions requires moving from laboratory prototypes to chronic clinical systems that support thousands to millions of electrodes, several millimeters to centimeters deep beneath the brain surface, under strict heating and size limits. Almost every clinically relevant implant therefore operates in a weakly coupled regime, with coupling coefficients of $10^{-3}$ to $10^{-1}$ across centimetres of lossy tissue. In this regime, the wireless channel sets the limits of power-transfer efficiency, communication bandwidth, and energy per bit. We review the recent progress of bidirectional wireless links across inductive, mid-field, RF, ultrasonic, magnetoelectric, optical, UWB, and electro-quasistatic modalities, and benchmark them against the clinical axes of depth, size, and data rate. Within an approximately 10 mW communication budget set by the approximately $1^\circ$C tissue-heating ceiling, narrowband high-Q links are well suited for power transfer and low-speed data, but at 1-10 nJ/b cannot reach the greater than 10 Mbps to tens of Gbps uplinks that thousand- to million-channel interfaces demand, even with aggressive on-implant compression. This calls for sub-10 pJ/b and ultimately sub-1 pJ/b wireless links, where wideband techniques, such as ultra-wideband (UWB) and brain-channel communication (BCC), are suitable. We close with a quantitative framework for analyzing such wireless links and a co-design roadmap across electromagnetics, circuits, packaging, security, and regulation, toward secure, networked, million-channel brain interfaces.

==> do_not_use/bibitem_bibliography.tex <==
\begin{thebibliography}{999}
\bibitem[1]{ref1} Hochberg, L. R. et al. Neuronal ensemble control of prosthetic devices by a human with tetraplegia. \emph{Nature} \textbf{442}, 164--171 (2006).

\bibitem[2]{ref2} Collinger, J. L. et al. High-performance neuroprosthetic control by an individual with tetraplegia. \emph{Lancet} \textbf{381}, 557--564 (2013).

\bibitem[3]{ref3} Willett, F. R., Avansino, D. T., Hochberg, L. R., Henderson, J. M. \& Shenoy, K. V. High-performance brain-to-text communication via handwriting. \emph{Nature} \textbf{593}, 249--254 (2021).

\bibitem[4]{ref4} Willett, F. R. et al. A high-performance speech neuroprosthesis. \emph{Nature} \textbf{620}, 1031--1036 (2023).

\bibitem[5]{ref5} Metzger, S. L. et al. A high-performance neuroprosthesis for speech decoding and avatar control. \emph{Nature} \textbf{620}, 1037--1046 (2023).

\bibitem[6]{ref6} Card, N. S. et al. An accurate and rapidly calibrating speech neuroprosthesis. \emph{N. Engl. J. Med.} \textbf{391}, 609--618 (2024).

\bibitem[7]{ref7} Kunz, E. M. et al. Decoding inner speech from motor cortex. \emph{Cell} \textbf{188}, 5132--5147 (2025).

\bibitem[8]{ref8} Mitchell, P. et al. Assessment of safety of a fully implanted endovascular brain--computer interface for severe paralysis in 4 patients: the SWITCH study. \emph{JAMA Neurol.} \textbf{80}, 270--278 (2023).

\bibitem[9]{ref9} Oxley, T. J. et al. Motor neuroprosthesis implanted with neurointerventional surgery improves capacity for activities of daily living tasks in severe paralysis: first in-human experience. \emph{J. NeuroInterv. Surg.} \textbf{13}, 102--108 (2021).

\bibitem[10]{ref10} Musk, E. \& Neuralink. An integrated brain--machine interface platform with thousands of channels. \emph{J. Med. Internet Res.} \textbf{21}, e16194 (2019).

\bibitem[11]{ref11} Simeral, J. D. et al. Home use of a percutaneous wireless intracortical brain--computer interface by individuals with tetraplegia. \emph{IEEE Trans. Biomed. Eng.} \textbf{68}, 2313--2325 (2021).

\bibitem[12]{ref12} Sahasrabuddhe, K. et al. The Argo: a high-channel-count recording system for neural recording in vivo. \emph{J. Neural Eng.} \textbf{18}, 015002 (2021). [Paradromics]

\bibitem[13]{ref13} Chiang, C.-H. et al. A high-channel-count, conformal, microECoG array for recording and stimulating cortical activity. \emph{Sci. Transl. Med.} \textbf{12}, eaay4682 (2020). [Precision-related lineage]

\bibitem[14]{ref14} Steinmetz, N. A. et al. Neuropixels 2.0: a miniaturized high-density probe for stable, long-term brain recordings. \emph{Science} \textbf{372}, eabf4588 (2021).

\bibitem[15]{ref15} Lopez, C. M. et al. A 966-electrode neural probe with 384 configurable channels in 0.13-$\mu$m SOI CMOS. \emph{IEEE J. Solid-State Circuits} \textbf{52}, 510--522 (2017).

\bibitem[16]{ref16} Borton, D. A., Yin, M., Aceros, J. \& Nurmikko, A. An implantable wireless neural interface for recording cortical circuit dynamics in moving primates. \emph{J. Neural Eng.} \textbf{10}, 026010 (2013).

\bibitem[17]{ref17} Yin, M. et al. Wireless neurosensor for full-spectrum electrophysiology recordings during free behavior. \emph{Neuron} \textbf{84}, 1170--1182 (2014).

\bibitem[18]{ref18} Schwarz, D. A. et al. Chronic, wireless recordings of large-scale brain activity in freely moving rhesus monkeys. \emph{Nat. Methods} \textbf{11}, 670--676 (2014).

\bibitem[19]{ref19} Harrison, R. R. et al. A low-power integrated circuit for a wireless 100-electrode neural recording system. \emph{IEEE J. Solid-State Circuits} \textbf{42}, 123--133 (2007).

\bibitem[20]{ref20} Ho, J. S. et al. Wireless power transfer to deep-tissue microimplants. \emph{Proc. Natl Acad. Sci. USA} \textbf{111}, 7974--7979 (2014).

\bibitem[21]{ref21} Kim, S., Ho, J. S. \& Poon, A. S. Y. Midfield wireless powering of subwavelength autonomous devices. \emph{Phys. Rev. Lett.} \textbf{110}, 203905 (2013).

\bibitem[22]{ref22} Poon, A. S. Y., O'Driscoll, S. \& Meng, T. H. Optimal frequency for wireless power transmission into dispersive tissue. \emph{IEEE Trans. Antennas Propag.} \textbf{58}, 1739--1750 (2010).

\bibitem[23]{ref23} Seo, D. et al. Wireless recording in the peripheral nervous system with ultrasonic neural dust. \emph{Neuron} \textbf{91}, 529--539 (2016).

\bibitem[24]{ref24} Seo, D., Carmena, J. M., Rabaey, J. M., Alon, E. \& Maharbiz, M. M. Neural dust: an ultrasonic, low power solution for chronic brain--machine interfaces. Preprint at https://arxiv.org/abs/1307.2196 (2013).

\bibitem[25]{ref25} Piech, D. K. et al. A wireless millimetre-scale implantable neural stimulator with ultrasonically powered bidirectional communication. \emph{Nat. Biomed. Eng.} \textbf{4}, 207--222 (2020).

\bibitem[26]{ref26} Ghanbari, M. M. et al. A sub-mm$^{3}$ ultrasonic free-floating implant for multi-mote neural recording. \emph{IEEE J. Solid-State Circuits} \textbf{54}, 3017--3030 (2019).

\bibitem[27]{ref27} Charthad, J. et al. A mm-sized wireless implantable device for electrical stimulation of peripheral nerves. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{12}, 257--270 (2018).

\bibitem[28]{ref28} Yu, Z. et al. MagNI: a magnetoelectrically powered and controlled wireless neurostimulating implant. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{14}, 1241--1252 (2020).

\bibitem[29]{ref29} Singer, A. et al. Magnetoelectric materials for miniature, wireless neural stimulation at therapeutic frequencies. \emph{Neuron} \textbf{107}, 631--643 (2020).

\bibitem[30]{ref30} Alrashdan, F. T. et al. Wearable wireless power systems for 'ME-BIT' magnetoelectric-powered bio implants. \emph{J. Neural Eng.} \textbf{18}, 045011 (2021).

\bibitem[31]{ref31} Kim, A. et al. An implantable ultrasonically-powered micro-light-source ($\mu$Light) for photodynamic therapy. \emph{Sci. Rep.} \textbf{9}, 1395 (2019).

\bibitem[32]{ref32} Khalifa, A. et al. The microbead: a 0.009 mm$^{3}$ implantable wireless neural stimulator. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{13}, 971--985 (2019).

\bibitem[33]{ref33} Lee, J. et al. Neural recording and stimulation using wireless networks of microimplants. \emph{Nat. Electron.} \textbf{4}, 604--614 (2021).

\bibitem[34]{ref34} Chen, Y.-P. et al. An injectable 64 nW ECG mixed-signal SoC in 65 nm for arrhythmia monitoring. \emph{IEEE J. Solid-State Circuits} \textbf{50}, 375--390 (2015).

\bibitem[35]{ref35} Muller, R. et al. A minimally invasive 64-channel wireless $\mu$ECoG implant. \emph{IEEE J. Solid-State Circuits} \textbf{50}, 344--359 (2015).

\bibitem[36]{ref36} Biederman, W. et al. A 4.78 mm$^{2}$ fully-integrated neuromodulation SoC combining 64 acquisition channels with digital compression and simultaneous dual stimulation. \emph{IEEE J. Solid-State Circuits} \textbf{50}, 1038--1047 (2015).

\bibitem[37]{ref37} Yeon, P. et al. A 100Mb/s --32dB sensitivity fully synchronous wireless data telemetry IC for high-channel-count neural recordings. In \emph{Symp. VLSI Circuits} C234--C235 (2017).

\bibitem[38]{ref38} Mirbozorgi, S. A. et al. A single-chip full-duplex high-speed transceiver for multi-site stimulating and recording neural implants. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{10}, 643--653 (2016).

\bibitem[39]{ref39} Wang, P.-H. P. et al. A 6.1-nJ/bit energy-harvesting Bluetooth low-energy transmitter using DCO duty cycling and adaptive matching. \emph{IEEE J. Solid-State Circuits} \textbf{53}, 3071--3082 (2018).

\bibitem[40]{ref40} Park, S.-Y., Cho, J., Lee, K. \& Yoon, E. A PVDF-based 100Mb/s transcutaneous IR-UWB link for high-bandwidth implantable medical devices. In \emph{IEEE Custom Integr. Circuits Conf.} 1--4 (2017).

\bibitem[41]{ref41} Chen, Y.-P. et al. A 1.66 Gb/s and 5.8 pJ/b transcutaneous IR-UWB telemetry system with hybrid OOK/PPM modulation for wireless neural recording. \emph{IEEE J. Solid-State Circuits} \textbf{59}, 2470--2483 (2024).

\bibitem[42]{ref42} Lee, S. et al. A 6--9 GHz CMOS IR-UWB transmitter with hybrid pulse modulation. \emph{IEEE Trans. Microw. Theory Tech.} \textbf{70}, 4710--4721 (2022).

\bibitem[43]{ref43} Mercier, P. P., Daly, D. C. \& Chandrakasan, A. P. An energy-efficient all-digital UWB transmitter employing dual capacitively-coupled pulse-shaping drivers. \emph{IEEE J. Solid-State Circuits} \textbf{44}, 1679--1688 (2009).

\bibitem[44]{ref44} Wentzloff, D. D. \& Chandrakasan, A. P. A 47 pJ/pulse 3.1-to-5 GHz all-digital UWB transmitter in 90 nm CMOS. In \emph{IEEE ISSCC Dig. Tech. Papers} 118--119 (2007).

\bibitem[45]{ref45} Maity, S. et al. BodyWire: a 6.3-pJ/b 30-Mb/s --30-dB SIR-tolerant broadband interference-robust human body communication transceiver using time-domain interference rejection. \emph{IEEE J. Solid-State Circuits} \textbf{54}, 2892--2906 (2019).

\bibitem[46]{ref46} Chatterjee, B. et al. Bio-physical modeling, characterization, and optimization of electro-quasistatic human body communication. \emph{IEEE Trans. Biomed. Eng.} \textbf{66}, 1791--1802 (2019).

\bibitem[47]{ref47} Nath, M., Maity, S. \& Sen, S. Toward understanding the return path capacitance in capacitive human body communication. \emph{IEEE Trans. Circuits Syst. II} \textbf{67}, 1879--1883 (2020).

\bibitem[48]{ref48} Modak, N., Nath, M., Chatterjee, B., Maity, S. \& Sen, S. Bio-physical modeling of galvanic human body communication in electro-quasistatic regime. \emph{IEEE Trans. Biomed. Eng.} \textbf{69}, 3717--3727 (2022).

\bibitem[49]{ref49} Maity, S., Mojabe, K. \& Sen, S. Characterization of human body forward path loss and variability effects in voltage-mode HBC. \emph{IEEE Microw. Wirel. Compon. Lett.} \textbf{28}, 266--268 (2018).

\bibitem[50]{ref50} Das, D., Maity, S., Chatterjee, B. \& Sen, S. Enabling covert body area network using electro-quasistatic human body communication. \emph{Sci. Rep.} \textbf{9}, 4160 (2019).

\bibitem[51]{ref51} Chatterjee, B., Cao, N., Raychowdhury, A. \& Sen, S. Context-aware intelligence in resource-constrained IoT nodes: opportunities and challenges. \emph{IEEE Des. Test} \textbf{36}, 7--40 (2019).

\bibitem[52]{ref52} Avlani, S. et al. A 100KHz--1GHz termination-dependent human body communication channel measurement using miniaturized wearable devices. In \emph{Design, Automation \& Test in Europe} 1117--1120 (2020).

\bibitem[53]{ref53} Cao, N. et al. A 0.2-mW 88\%-PCE buck converter and a co-designed body-coupled receiver for energy-harvesting body-area applications. \emph{IEEE J. Solid-State Circuits} \textbf{53}, 3501--3513 (2018).

\bibitem[54]{ref54} Chatterjee, B. et al. A 1.15 $\mu$W 5.54 mm$^{3}$ implant with a bidirectional neural sensor and stimulator SoC utilizing bi-phasic quasi-static brain communication achieving 6 kbps--10 Mbps uplink with compressive sensing and RO-PUF based collision avoidance. In \emph{IEEE Symp. VLSI Circuits} 1--2 (2021).

\bibitem[54a]{ref54a} Chatterjee, B., Mohseni, P. \& Sen, S. Bioelectronic sensor nodes for the Internet of Bodies. \emph{Annu. Rev. Biomed. Eng.} \textbf{25}, 101--129 (2023).

\bibitem[55]{ref55} Sen, S. SocialHBC: social networking and secure authentication using interference-robust human body communication. In \emph{Proc. ACM Int. Symp. Low Power Electronics and Design} 34--39 (2016).

\bibitem[56]{ref56} Maity, S., He, M., Nath, M., Das, D., Chatterjee, B. \& Sen, S. Bio-physical modeling, characterization, and optimization of electro-quasistatic human body communication. Preprint at https://arxiv.org/abs/1805.05200 (2018).

\bibitem[57]{ref57} Wegmueller, M. S. et al. Signal transmission by galvanic coupling through the human body. \emph{IEEE Trans. Instrum. Meas.} \textbf{59}, 963--969 (2010).

\bibitem[58]{ref58} Park, J. \& Mercier, P. P. Magnetic human body communication. In \emph{Proc. IEEE EMBC} 1841--1844 (2015).

\bibitem[59]{ref59} Mercier, P. P. et al. Energy-autonomous wireless body sensors. \emph{Nat. Electron.} \textbf{2}, 514--522 (2019).

\bibitem[60]{ref60} Zhang, H. \& Mercier, P. P. A 9.7 pJ/b human body communication transceiver with adaptive equalization. \emph{IEEE J. Solid-State Circuits} \textbf{56}, 2864--2876 (2021).

\bibitem[61]{ref61} Kim, J. et al. A 0.5-V sub-microwatt CMOS image sensor with reset-gate-less active pixel circuitry. \emph{IEEE J. Solid-State Circuits} \textbf{54}, 2299--2308 (2019).

\bibitem[62]{ref62} Mahmoud, M. et al. Empirical and statistical models for the in-body path loss in MICS band. \emph{IEEE Antennas Wirel. Propag. Lett.} \textbf{18}, 1064--1068 (2019).

\bibitem[63]{ref63} Kurup, D., Joseph, W., Vermeeren, G. \& Martens, L. In-body path loss model for homogeneous human muscle, brain, fat, and skin tissues. In \emph{Proc. 4th Eur. Conf. Antennas Propag.} 1--5 (2010).

\bibitem[64]{ref64} Sayrafian-Pour, K., Yang, W.-B., Hagedorn, J., Terrill, J. \& Yazdandoost, K. Y. A statistical path loss model for medical implant communication channels. In \emph{IEEE PIMRC} 2995--2999 (2009).

\bibitem[65]{ref65} IEEE Standards Association. \emph{IEEE Std C95.1-2019: IEEE Standard for Safety Levels with Respect to Human Exposure to Electric, Magnetic, and Electromagnetic Fields, 0 Hz to 300 GHz} (IEEE, 2019).

\bibitem[66]{ref66} International Commission on Non-Ionizing Radiation Protection. Guidelines for limiting exposure to electromagnetic fields (100 kHz to 300 GHz). \emph{Health Phys.} \textbf{118}, 483--524 (2020).

\bibitem[67]{ref67} Lazzi, G. Thermal effects of bioimplants. \emph{IEEE Eng. Med. Biol. Mag.} \textbf{24}, 75--81 (2005).

\bibitem[68]{ref68} Kim, S., Tathireddy, P., Normann, R. A. \& Solzbacher, F. Thermal impact of an active 3-D microelectrode array implanted in the brain. \emph{IEEE Trans. Neural Syst. Rehabil. Eng.} \textbf{15}, 493--501 (2007).

\bibitem[69]{ref69} Federal Communications Commission. \emph{Medical Device Radiocommunications Service (MedRadio): Rules and Regulations} (FCC, 2024).

\bibitem[70]{ref70} Yakovlev, A., Kim, S. \& Poon, A. Implantable biomedical devices: wireless powering and communication. \emph{IEEE Commun. Mag.} \textbf{50}, 152--159 (2012).

\bibitem[71]{ref71} Agarwal, K., Jegadeesan, R., Guo, Y.-X. \& Thakor, N. V. Wireless power transfer strategies for implantable bioelectronics. \emph{IEEE Rev. Biomed. Eng.} \textbf{10}, 136--161 (2017).

\bibitem[72]{ref72} Lazaro, A., Villarino, R. \& Girbau, D. A survey of NFC sensors based on energy harvesting for IoT applications. \emph{Sensors} \textbf{18}, 3746 (2018).

\bibitem[73]{ref73} RamRakhyani, A. K., Mirabbasi, S. \& Chiao, M. Design and optimization of resonance-based efficient wireless power delivery systems for biomedical implants. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{5}, 48--63 (2011).

\bibitem[74]{ref74} Jow, U.-M. \& Ghovanloo, M. Design and optimization of printed spiral coils for efficient transcutaneous inductive power transmission. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{1}, 193--202 (2007).

\bibitem[75]{ref75} Mirbozorgi, S. A., Bahrami, H., Sawan, M. \& Gosselin, B. A smart cage with uniform wireless power distribution in 3D for enabling long-term experiments with freely moving animals. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{10}, 424--434 (2016).

\bibitem[76]{ref76} Chen, X. et al. Microwave-based wireless power transfer to deep brain implants for closed-loop neuromodulation. \emph{Nat. Biomed. Eng.} \textbf{6}, 706--716 (2022).

\bibitem[77]{ref77} Iqbal, A. et al. A review of in-body biotelemetry devices: implantables, ingestibles, and injectables. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{17}, 1--24 (2023).

\bibitem[78]{ref78} Yousaf, M., Mehmood, M. \& Riaz, A. Compact and efficient antennas for implantable medical devices: a survey. \emph{IEEE Access} \textbf{10}, 88820--88846 (2022).

\bibitem[79]{ref79} So, J. H., Mercier, P. P. et al. An RF-ultrasound relay for adaptive wireless powering across air-tissue interfaces. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{16}, 1063--1075 (2022).

\bibitem[80]{ref80} Mariello, M. et al. Soft and flexible bioelectronic micro-systems for electronically controlled drug delivery. \emph{Adv. Healthc. Mater.} \textbf{11}, 2102297 (2022).

\bibitem[81]{ref81} Liu, Y. et al. Soft and elastic hydrogel-based microelectronics for localized low-voltage neuromodulation. \emph{Nat. Biomed. Eng.} \textbf{3}, 58--68 (2019).

\bibitem[82]{ref82} Park, S. I. et al. Soft, stretchable, fully implantable miniaturized optoelectronic systems for wireless optogenetics. \emph{Nat. Biotechnol.} \textbf{33}, 1280--1286 (2015).

\bibitem[83]{ref83} Burton, A. et al. Wireless, battery-free subdermally implantable photometry systems for chronic recording of neural dynamics. \emph{Proc. Natl Acad. Sci. USA} \textbf{117}, 2835--2845 (2020).

\bibitem[84]{ref84} Won, S. M. et al. Wireless and battery-free technologies for neuroengineering. \emph{Nat. Biomed. Eng.} \textbf{5}, 405--423 (2021).

\bibitem[85]{ref85} Hong, G. \& Lieber, C. M. Novel electrode technologies for neural recordings. \emph{Nat. Rev. Neurosci.} \textbf{20}, 330--345 (2019).

\bibitem[86]{ref86} Patel, S. R. \& Lieber, C. M. Precision electronic medicine in the brain. \emph{Nat. Biotechnol.} \textbf{37}, 1007--1012 (2019).

\bibitem[87]{ref87} Topalovic, U. et al. A wearable platform for closed-loop stimulation and recording of single-neuron and local field potential activity in freely moving humans. \emph{Nat. Neurosci.} \textbf{26}, 517--527 (2023).

\bibitem[88]{ref88} Khalifa, A. et al. A neural interface circuit and microelectrode array system for high-density wireless electrophysiology. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{17}, 1057--1071 (2023).

\bibitem[89]{ref89} Sharma, P. et al. A high-channel-count fully integrated head-mounted $\mu$ECoG platform supporting 5,376 channels. \emph{Nat. Electron.} \textbf{7}, 870--881 (2024).

\bibitem[90]{ref90} Ho, J. S., Kim, S. \& Poon, A. S. Y. Midfield wireless powering for implantable systems. \emph{Proc. IEEE} \textbf{101}, 1369--1378 (2013).

\bibitem[91]{ref91} Khalifa, A. et al. The microbead: a highly miniaturized wirelessly powered implantable neural stimulating system. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{12}, 521--531 (2018).

\bibitem[92]{ref92} Lyu, H. et al. A 430-MHz wirelessly powered implantable pulse generator with intensity/rate control and sub-1 $\mu$A quiescent current consumption. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{13}, 180--190 (2019).

\bibitem[93]{ref93} Lee, B., Jia, Y., Mirbozorgi, S. A. \& Ghovanloo, M. An inductive power and data telemetry subsystem with fast transient low dropout regulator. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{13}, 1015--1024 (2019).

\bibitem[94]{ref94} Kilinc, E. G., Conus, G., Weber, C., Kawkabani, B., Maloberti, F. \& Dehollain, C. A system for wireless power transfer and data communication of long-term bio-monitoring. \emph{IEEE Sens. J.} \textbf{15}, 6559--6569 (2015).

\bibitem[95]{ref95} Sharma, A., Chong, G., Heng, C.-H. \& Lian, Y. A 32 ch fully implantable neural recording SoC with wireless power and data link. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{15}, 1230--1241 (2021).

\bibitem[96]{ref96} Lee, K., Park, J. \& Ghovanloo, M. A novel power and data transmission method for wireless neural recording systems. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{16}, 1102--1114 (2022).

\bibitem[97]{ref97} Yin, M., Borton, D. A., Aceros, J., Patterson, W. R. \& Nurmikko, A. V. A 100-channel hermetically sealed implantable device for chronic wireless neurosensing applications. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{7}, 115--128 (2013).

\bibitem[98]{ref98} Chen, K., Yang, Z., Hoang, L., Weiland, J., Humayun, M. \& Liu, W. An integrated 256-channel epiretinal prosthesis. \emph{IEEE J. Solid-State Circuits} \textbf{45}, 1946--1956 (2010).

\bibitem[99]{ref99} Lo, Y.-K. et al. A fully integrated wireless SoC for motor function recovery after spinal cord injury. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{11}, 497--509 (2017).

\bibitem[100]{ref100} Mahmoud, A. et al. A 0.6V 12 $\mu$W implantable closed-loop neuromodulation SoC. In \emph{IEEE ISSCC} 1--3 (2024).

\bibitem[101]{ref101} Sun, F.-W. et al. A 6.78 MHz simultaneous wireless information and power transfer system for biomedical implants. \emph{IEEE J. Solid-State Circuits} \textbf{57}, 3486--3497 (2022).

\bibitem[102]{ref102} Jia, Y., Khan, W., Lee, B., Fan, B., Madi, F. \& Ghovanloo, M. Wireless opto-electro neural interface for experiments with small freely behaving animals. \emph{J. Neural Eng.} \textbf{15}, 046032 (2018).

\bibitem[103]{ref103} Soltani, N. et al. A neural-stimulating SoC with on-chip patient-specific charge balancing. \emph{IEEE J. Solid-State Circuits} \textbf{57}, 134--149 (2022).

\bibitem[104]{ref104} Jia, Y. et al. A mm-sized free-floating wirelessly powered implantable optical stimulating SoC. In \emph{IEEE ISSCC Dig. Tech. Papers} 468--470 (2018).

\bibitem[105]{ref105} Charthad, J., Weber, M. J., Chang, T. C. \& Arbabian, A. A mm-sized implantable medical device (IMD) with ultrasonic power transfer and a hybrid bi-directional data link. \emph{IEEE J. Solid-State Circuits} \textbf{50}, 1741--1753 (2015).

\bibitem[106]{ref106} Sonmezoglu, S., Fineman, J. R., Maltepe, E. \& Maharbiz, M. M. Monitoring deep-tissue oxygenation with a millimeter-scale ultrasonic implant. \emph{Nat. Biotechnol.} \textbf{39}, 855--864 (2021).

\bibitem[107]{ref107} Shi, C., Costa, T., Elloian, J., Zhang, Y. \& Shepard, K. L. A 0.065-mm$^{3}$ monolithically-integrated ultrasonic wireless sensing mote for real-time physiological temperature monitoring. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{14}, 412--424 (2020).

\bibitem[108]{ref108} Weber, M. J., Yoshihara, Y., Sawaby, A., Charthad, J., Chang, T. C. \& Arbabian, A. A miniaturized single-transducer implantable pressure sensor with time-multiplexed ultrasonic data and power links. \emph{IEEE J. Solid-State Circuits} \textbf{53}, 1089--1101 (2018).

\bibitem[109]{ref109} Vasli, B. \& Arbabian, A. Multi-mode adaptive ultrasonic powering for deep-tissue mm-sized implants. \emph{IEEE J. Solid-State Circuits} \textbf{57}, 1234--1247 (2022).

\bibitem[110]{ref110} Singer, A. \& Robinson, J. T. Wireless power delivery techniques for miniature implantable bioelectronics. \emph{Adv. Healthc. Mater.} \textbf{10}, 2100664 (2021).

\bibitem[111]{ref111} Yu, Z. et al. An 8.2-mm$^{3}$ implantable neurostimulator with magnetoelectric power and data transfer. In \emph{IEEE ISSCC Dig. Tech. Papers} 510--512 (2020).

\bibitem[112]{ref112} Burton, A. R. et al. Magnetoelectrics for implantable bioelectronics: progress to date. \emph{Adv. Funct. Mater.} \textbf{34}, 2316030 (2024).

\bibitem[113]{ref113} Mei, H. \& Irazoqui, P. P. Miniaturizing wireless implants. \emph{Nat. Biotechnol.} \textbf{32}, 1008--1010 (2014).

\bibitem[114]{ref114} Park, S. Y. et al. A 64-channel chip-scale neural recording IC employing reverse telemetry. \emph{IEEE J. Solid-State Circuits} \textbf{57}, 1234--1245 (2022).

\bibitem[115]{ref115} Bos, R. et al. A 31.6 $\mu$W BLE-conformant transmitter using event-driven RF data path. \emph{IEEE J. Solid-State Circuits} \textbf{57}, 750--762 (2022).

\bibitem[116]{ref116} Wang, P.-H. P., Mercier, P. P. et al. A near-zero-power wake-up receiver achieving -80 dBm sensitivity via a passive matching network. \emph{IEEE J. Solid-State Circuits} \textbf{55}, 1640--1652 (2020).

\bibitem[117]{ref117} Roberts, N. E. et al. A 236 nW -56.5 dBm-sensitivity Bluetooth Low Energy wakeup receiver with energy harvesting. \emph{IEEE Trans. Circuits Syst. I} \textbf{63}, 1934--1946 (2016).

\bibitem[118]{ref118} Mercier, P. P. \& Chandrakasan, A. P. (Eds) \emph{Ultra-Low-Power Short-Range Radios} (Springer, 2015).

\bibitem[119]{ref119} Avlani, S. et al. A 4.5pJ/bit human-body-channel transceiver for IoT applications. In \emph{IEEE Custom Integr. Circuits Conf.} 1--4 (2020).

\bibitem[120]{ref120} Mai, S. et al. A 30Mbps adaptively modulated transcutaneous data telemetry system using a single inductive link for next-generation neural prostheses. In \emph{IEEE ISSCC Dig. Tech. Papers} 318--319 (2020).

\bibitem[121]{ref121} Lim, J. et al. A 0.19$\times$0.17 mm$^{2}$ wireless neural recording IC for motor prediction with near-infrared-based power and data telemetry. In \emph{IEEE ISSCC Dig. Tech. Papers} 416--418 (2020).

\bibitem[122]{ref122} Kassiri, H. et al. Closed-loop neurostimulator with on-chip seizure detection for chronic implantation. \emph{IEEE J. Solid-State Circuits} \textbf{52}, 2793--2809 (2017).

\bibitem[123]{ref123} Reza, A. et al. Spike sorting on-chip: a low-power solution for high-channel-count neural recording. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{15}, 1095--1109 (2021).

\bibitem[124]{ref124} Valencia, D. \& Alimohammad, A. Compression of neural data using deep learning. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{15}, 1305--1314 (2021).

\bibitem[125]{ref125} Aprile, C., Wuthrich, K., Baldassarre, L., Brunelli, D., Cevher, V. \& Leblebici, Y. Adaptive learning-based compressive sampling for low-power wireless implants. \emph{IEEE Trans. Circuits Syst. I} \textbf{65}, 3578--3590 (2018).

\bibitem[126]{ref126} Karimi, S., Mirbozorgi, S. A., Babakhani, A. \& Gosselin, B. CMOS neural recording front-ends with energy-efficient compression. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{17}, 540--554 (2023).

\bibitem[127]{ref127} Halperin, D. et al. Pacemakers and implantable cardiac defibrillators: software radio attacks and zero-power defenses. In \emph{IEEE Symp. Security and Privacy} 129--142 (2008).

\bibitem[128]{ref128} Marin, E., Singelée, D., Garcia, F. D., Chothia, T., Willems, R. \& Preneel, B. On the security of implantable medical devices: a survey. \emph{IEEE Internet Things J.} \textbf{8}, 8546--8562 (2021).

\bibitem[129]{ref129} Ghosh, A., Maity, A. \& Sen, S. PowerScout: security-oriented power delivery network modeling for side-channel vulnerability analysis. \emph{IEEE Des. Test} \textbf{40}, 7--18 (2023).

\bibitem[130]{ref130} Chatterjee, B. et al. A post-quantum secure communication protocol with ultra-low power for implantable medical devices. \emph{IEEE Trans. Biomed. Circuits Syst.} \textbf{18}, in press (2025).

\bibitem[131]{ref131} Mahmoud, A., Hu, X. S. et al. Hardware-aware lightweight authentication for low-power neural implants. \emph{IEEE Trans. Very Large Scale Integr. (VLSI) Syst.} \textbf{31}, 1100--1112 (2023).

\bibitem[132]{ref132} NIST. \emph{Post-Quantum Cryptography Standardization: Final Standards FIPS 203, 204, 205} (NIST, 2024).

\bibitem[133]{ref133} Halperin, D. \& Kohno, T. Electronic medical implants: privacy and security threats. In \emph{Proc. ACM CCS Workshop on Implantable Medical Devices} (2010).

\bibitem[134]{ref134} ARPA-H. \emph{Networked Wireless Implants Initiative,   Program Overview} (ARPA-H, 2024).

\bibitem[135]{ref135} DARPA. \emph{Next-Generation Nonsurgical Neurotechnology (N3) Program} (DARPA, 2023).

\bibitem[136]{ref136} Bouton, C. E. et al. Restoring cortical control of functional movement in a human with quadriplegia. \emph{Nature} \textbf{533}, 247--250 (2016).

\bibitem[137]{ref137} Ajiboye, A. B. et al. Restoration of reaching and grasping movements through brain-controlled muscle stimulation in a person with tetraplegia: a proof-of-concept demonstration. \emph{Lancet} \textbf{389}, 1821--1830 (2017).

\bibitem[138]{ref138} Anumanchipalli, G. K., Chartier, J. \& Chang, E. F. Speech synthesis from neural decoding of spoken sentences. \emph{Nature} \textbf{568}, 493--498 (2019).

\bibitem[139]{ref139} Moses, D. A. et al. Neuroprosthesis for decoding speech in a paralyzed person with anarthria. \emph{N. Engl. J. Med.} \textbf{385}, 217--227 (2021).

\bibitem[140]{ref140} Hong, G., Yang, X., Zhou, T. \& Lieber, C. M. Mesh electronics: a new paradigm for tissue-like brain probes. \emph{Curr. Opin. Neurobiol.} \textbf{50}, 33--41 (2018).

\bibitem[141]{ref141} Robinson, J. T. et al. Vision for a nationwide brain-computer interface initiative. \emph{Cell} \textbf{187}, 815--825 (2024).

\bibitem[142]{ref142} Sen, S., Maity, S. \& Das, D. The body is the network: to safeguard sensitive data, turn flesh and tissue into a secure wireless channel. \emph{IEEE Spectr.} \textbf{57}, 44--49 (2020).

\bibitem[143]{ref143} Sen, S. Invited: context-aware energy-efficient communication for IoT sensor nodes. In \emph{Proc. ACM/IEEE Des. Autom. Conf.} 1--6 (2016).

\bibitem[144]{ref144} Chatterjee, B., Krishnamurthy, A., Mohseni, P. \& Sen, S. Toward sub-microwatt brain implants: bidirectional bi-phasic quasi-static brain communication. \emph{IEEE Solid-State Circuits Mag.} \textbf{15}, 30--45 (2023).

\bibitem[145]{ref145} Tsai, T.-H. et al. A 32-channel intracortical neural recording SoC with on-chip spike-sorting and PWM-based ultra-wideband output. \emph{IEEE J. Solid-State Circuits} \textbf{57}, 2999--3013 (2022).

\bibitem[146]{ref146} Won, S. M., Cai, L., Gutruf, P. \& Rogers, J. A. Emerging modalities and implantable technologies for neuromodulation. \emph{Cell} \textbf{183}, 1--17 (2020).

\bibitem[147]{ref147} Wang, P. M. et al. Closed-loop wireless implantable platform for intracranial pressure regulation. \emph{Nat. Biomed. Eng.} \textbf{8}, 1175--1187 (2024).

\bibitem[148]{ref148} Tetzlaff, T. et al. AI-on-implant: neural-network inference for closed-loop neuromodulation under microwatt budgets. \emph{Nat. Electron.} \textbf{8}, 425--438 (2025).

\bibitem[149]{ref149} Tang, X. et al. Highly miniaturized, battery-free, wireless soft implant for chronic monitoring of intracranial pressure and temperature. \emph{Sci. Adv.} \textbf{9}, eadf2347 (2023).

\bibitem[150]{ref150} Robinson, J. T., Yang, K. et al. A mid-field powered, low-power wireless brain implant for chronic recording in freely-behaving primates. \emph{Nat. Electron.} in press (2026).
\end{thebibliography}

==> tables/table0_tissue_stack.tex <==
{
{\fontsize{8pt}{10pt}\selectfont
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.95}
\setlength{\baselineskip}{0pt}
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}

\begin{longtable}{@{}p{3.0cm}P{2.0cm}p{5.5cm}p{2.8cm}@{}}
\caption{\textbf{Nine-layer brain-tissue stack used in the capacity framework.} Layer thicknesses are representative of an adult human at the skull vertex.}
\label{tab:tissue_stack}\\
\toprule
\textbf{Layer} & \textbf{$t$ (mm)} & \textbf{IT\textquotesingle IS~v5.0 entry} & \textbf{Group} \\
\midrule
Skin & 3.0 & Skin & Scalp \\
Fat & 2.5 & Fat (subcutaneous) & Scalp \\
\midrule
Outer cortical & 2.0 & Bone (Cortical) & Skull \\
Diploe & 4.0 & Bone (Cancellous) & Skull \\
Inner cortical & 1.5 & Bone (Cortical) & Skull \\
\midrule
Dura mater & 1.5 & Dura & CSF/meninges \\
CSF & 2.5 & Cerebrospinal Fluid & CSF/meninges \\
\midrule
Grey matter & 4.0 & Brain (Grey Matter) & Brain \\
White matter & 10.5 & Brain (White Matter) & Brain \\
\midrule
\textbf{Total} & \textbf{31.5} &  &  \\
\bottomrule
\end{longtable}
}
}


==> tables/table1a_wpt_chain.tex <==
{
{\fontsize{8pt}{5pt}\selectfont
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.80}
\setlength{\baselineskip}{0pt}
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}

\begin{longtable}{@{}P{1.1cm}P{1.6cm}P{1.3cm}P{1.8cm}P{1.5cm}P{1.5cm}P{1.9cm}P{1.9cm}p{2.5cm}@{}}
\caption{\textbf{WPT power chain at $d=30$\,mm, single-tissue phantom.} Paper-anchored values \cite{kiani_iscas25}. PTE, power transfer efficiency; $R_L$, optimal load resistance; $V_{\mathrm{oc}}$, open-circuit voltage at receiver.}
\label{tab:wpt_chain}\\
\toprule
\textbf{Mod.} & \textbf{Freq.} & \textbf{PTE (\%)} & \textbf{$P_{\mathrm{tx}}$ (mW)} & \textbf{$P_L$ (mW)} & \textbf{$R_L$ ($\Omega$)} & \textbf{$V_{L,\mathrm{pk}}$ (V)} & \textbf{$V_{\mathrm{oc}}$ (V)} & \textbf{Rx size} \\
\midrule
NIC & 33.5\,MHz & 4.000 & 192.5 & 7.70 & 220 & 1.3015 & 2.6031 & $\pi{\times}2.1^2{\times}5.8\,mm^3$ \\
US & 238\,kHz & 0.400 & 3887.5 & 15.55 & 3000 & 6.8301 & 13.6602 & $6.4{\times}2.3{\times}1.4$\,mm$^3$ \\
ME & 279.2\,kHz & 0.020 & 35000.0 & 7.00 & 7000 & 7.0000 & 14.0000 & $6.4{\times}2.3{\times}1.6$\,mm$^3$ \\
\bottomrule
\end{longtable}
}
}


==> tables/table1b_dl_snr.tex <==
{
{\fontsize{8pt}{5pt}\selectfont
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.80}
\setlength{\baselineskip}{0pt}
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}

\begin{longtable}{@{}P{1.3cm}P{1.0cm}P{2.0cm}P{1.5cm}P{2.1cm}P{2.1cm}p{3.8cm}@{}}
\caption{\textbf{Downlink channel SNR and Shannon capacity at $d = 10$, 20, 30\,mm.} $S_n = 5$\,nV\,$\sqrt{\mathrm{Hz}}^{-1}$. Cole-Cole tissue correction (IT\textquotesingle IS~v5.0). Matched: power-matched load; High-Z: high-impedance receiver ($V_L \approx V_\mathrm{oc}$).}
\label{tab:dl_snr}\\
\toprule
\textbf{Mod.} & \parbox[t]{\linewidth}{\centering\textbf{$d$}\\[2pt]{\scriptsize(mm)}} & \textbf{BW} & \parbox[t]{\linewidth}{\centering\textbf{SNR}\\[2pt]{\scriptsize(dB)}} & \parbox[t]{\linewidth}{\centering\textbf{$C_{\mathrm{match}}$}\\[2pt]{\scriptsize(Mbps)}} & \parbox[t]{\linewidth}{\centering\textbf{$C_{\mathrm{High\text{-}Z}}$}\\[2pt]{\scriptsize(Mbps)}} & \textbf{Limiting constraint} \\
\midrule
NIC & 10 & 418.8\,kHz & 122.7 & 17.07 & 17.91 & SAR, FCC \S1.1310 \\
 & 20 & 418.8\,kHz & 118.2 & 16.44 & 17.28 &  \\
 & 30 & 418.8\,kHz & 113.0 & 15.72 & 16.56 &  \\
\midrule
US & 10 & 47.6\,kHz & 139.0 & 2.197 & 2.292 & $I_{\mathrm{SPTA}}$, FDA Track~3 \\
 & 20 & 47.6\,kHz & 131.1 & 2.074 & 2.169 &  \\
 & 30 & 47.6\,kHz & 128.7 & 2.035 & 2.13 &  \\
\midrule
ME & 10 & 52.98\,kHz & 139.2 & 2.451 & 2.557 & DRL, IEEE C95.1 \\
 & 20 & 52.98\,kHz & 137.8 & 2.426 & 2.532 &  \\
 & 30 & 52.98\,kHz & 135.8 & 2.389 & 2.495 &  \\
\bottomrule
\end{longtable}
}
}


==> tables/table2a_cc_correction.tex <==
{
{\fontsize{8pt}{5pt}\selectfont
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.80}
\setlength{\baselineskip}{0pt}
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}

\begin{longtable}{@{}P{1.2cm}P{2.4cm}P{2.4cm}P{2.0cm}P{2.4cm}P{2.4cm}@{}}
\caption{\textbf{IT\textquotesingle IS~v5.0 tissue correction relative to single-tissue measurement phantom.} $\Delta > 0$: brain path more lossy than phantom.\\\textbf{NIC, ME} phantom: muscle equivalent; $\Delta$ absorption differences. \\\textbf{US} phantom: muscle equivalent; $\Delta$ represents acoustic \emph{interface reflection} losses and absorption differences.\\\textbf{BCC}: $\Delta_\mathrm{BCC}=0$; losses reported in \cite{ref144} for multi-layer stack.\\}
\label{tab:cc_correction}\\
\toprule
\textbf{Mod.} & \textbf{$\Delta_{\mathrm{scalp}}$ (dB)} & \textbf{$\Delta_{\mathrm{skull}}$ (dB)} & \textbf{$\Delta_{\mathrm{CSF}}$ (dB)} & \textbf{$\Delta_{\mathrm{brain}}$ (dB)} & \textbf{$\Delta_{\mathrm{tot}}$ (dB)} \\
\midrule
NIC & -0.23 & -0.37 & +0.15 & -0.49 & -0.94 \\
US & +0.22 & +5.25 & +1.83 & -0.05 & +7.25 \\
ME & -0.02 & -0.03 & +0.02 & -0.04 & -0.07 \\
BCC & +0.00 & +0.00 & +0.00 & +0.00 & +0.00 \\
\bottomrule
\end{longtable}
}
}


==> tables/table2b_alpha_layer.tex <==
{
{\fontsize{8pt}{5pt}\selectfont
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.80}
\setlength{\baselineskip}{0pt}
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}

\begin{longtable}{@{}P{2.8cm}P{1.2cm}P{1.8cm}P{1.8cm}P{1.8cm}P{1.8cm}P{1.8cm}@{}}
\caption{\textbf{Plane-wave and acoustic absorption coefficient per tissue layer ($\alpha$).}\\EM (NIC, ME, BCC, UWB): Cole-Cole dispersion~\cite{gabriel1996dielectric} evaluated at modality centre frequency using IT\textquotesingle IS~v5.0 model parameters; Acoustic (US): $\alpha_0 f^b$ power law~\cite{Duck1990}.}
\label{tab:alpha_layer}\\
\toprule
\textbf{Tissue} & \textbf{$t$ (mm)} & \textbf{33.5\,MHz} & \textbf{238\,kHz} & \textbf{279.2\,kHz} & \textbf{50\,MHz} & \textbf{4\,GHz} \\
\textbf{} & \textbf{} & \textbf{$\alpha$ (dB\,mm$^{-1}$)} & \textbf{$\alpha$ (dB\,mm$^{-1}$)} & \textbf{$\alpha$ (dB\,mm$^{-1}$)} & \textbf{$\alpha$ (dB\,mm$^{-1}$)} & \textbf{$\alpha$ (dB\,mm$^{-1}$)} \\
\midrule
Skin & 3.0 & 0.042 & 0.044 & 0.000 & 0.055 & 0.626 \\
SubcutFat & 2.5 & 0.020 & 0.008 & 0.002 & 0.023 & 0.254 \\
OuterCortBone & 2.0 & 0.017 & 0.113 & 0.001 & 0.020 & 0.733 \\
Diploe & 4.0 & 0.030 & 0.073 & 0.003 & 0.036 & 0.547 \\
InnerCortBone & 1.5 & 0.017 & 0.113 & 0.001 & 0.020 & 0.733 \\
Dura & 1.5 & 0.069 & 0.028 & 0.006 & 0.086 & 0.701 \\
CSF & 2.5 & 0.135 & 0.000 & 0.013 & 0.163 & 1.047 \\
GreyMatter & 4.0 & 0.050 & 0.002 & 0.003 & 0.063 & 0.733 \\
WhiteMatter & 10.5 & 0.035 & 0.012 & 0.002 & 0.045 & 0.733 \\
\midrule
\textbf{Total} $\alpha t$ (dB) &  & \textbf{1.363} & \textbf{1.015} & \textbf{0.100} & \textbf{1.692} & \textbf{21.555} \\
\bottomrule
\end{longtable}
}
}


==> tables/table2c_total_loss.tex <==
{
{\fontsize{8pt}{5pt}\selectfont
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.80}
\setlength{\baselineskip}{0pt}
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}

\begin{longtable}{@{}P{2.8cm}P{1.2cm}P{1.6cm}P{1.6cm}P{1.6cm}P{1.6cm}P{1.6cm}@{}}
\caption{\textbf{Total one-way tissue absorption $\alpha t$ per layer.} Product of Table~\ref{tab:alpha_layer} and layer thickness; plane-wave approximation.\\\textbf{NIC, ME, BCC}: Absorption only; negligible Fresnel reflections at tissue interfaces un 100\,Mhz range.\\\textbf{UWB}: Absorption only; Fresnel reflections at tissue interfaces totaling $4.27$\,dB added internally to the link budget.\\\textbf{US} acoustic bulk absorption only; interface reflection losses ($\approx$\,6--7\,dB, skull-dominated) are computed separately and summed in Table~\ref{tab:cc_correction}. }
\label{tab:total_loss}\\
\toprule
\textbf{Tissue} & \textbf{$t$ (mm)} & \textbf{NIC} & \textbf{US} & \textbf{ME} & \textbf{BCC} & \textbf{UWB} \\
\textbf{} & \textbf{} & \textbf{$\alpha t$ (dB)} & \textbf{$\alpha t$ (dB)} & \textbf{$\alpha t$ (dB)} & \textbf{$\alpha t$ (dB)} & \textbf{$\alpha t$ (dB)} \\
\midrule
Skin & 3.0 & 0.127 & 0.131 & 0.000 & 0.166 & 1.879 \\
SubcutFat & 2.5 & 0.049 & 0.020 & 0.005 & 0.058 & 0.634 \\
OuterCortBone & 2.0 & 0.033 & 0.226 & 0.002 & 0.039 & 1.465 \\
Diploe & 4.0 & 0.121 & 0.292 & 0.010 & 0.145 & 2.186 \\
InnerCortBone & 1.5 & 0.025 & 0.169 & 0.002 & 0.030 & 1.099 \\
Dura & 1.5 & 0.104 & 0.042 & 0.010 & 0.128 & 1.051 \\
CSF & 2.5 & 0.338 & 0.001 & 0.032 & 0.407 & 2.618 \\
GreyMatter & 4.0 & 0.198 & 0.007 & 0.013 & 0.251 & 2.930 \\
WhiteMatter & 10.5 & 0.368 & 0.128 & 0.026 & 0.468 & 7.692 \\
\midrule
\textbf{Total} (dB) &  & \textbf{1.363} & \textbf{1.015} & \textbf{0.100} & \textbf{1.692} & \textbf{21.555} \\
\bottomrule
\end{longtable}
}
}


==> tables/table3_uplink.tex <==
{
{\fontsize{8pt}{5pt}\selectfont
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.80}
\setlength{\baselineskip}{0pt}
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}

\begin{longtable}{@{}P{1.4cm}P{0.8cm}P{1.4cm}P{1.3cm}P{1.1cm}P{1.5cm}P{1.6cm}P{1.3cm}P{1.3cm}P{1.4cm}@{}}
\caption{\textbf{Uplink Shannon capacity for all five modalities at three implant depths.} $P_{\mathrm{UL,max}} = 3$\,mW; $S_n = 5$\,nV\,$\sqrt{\mathrm{Hz}}^{-1}$. $L_{\mathrm{tis}}$: absolute one-way tissue absorption and reflection losses. $L_{\mathrm{path}}$: geometric/coupling path loss $= 10\log_{10}(P_{\mathrm{tx}}/P_{\mathrm{rx,match}})-L_{\mathrm{tis}}$. }
\label{tab:uplink}\\
\toprule
\textbf{Mod.} & \parbox[t]{\linewidth}{\centering\textbf{$d$}\\[2pt]{\scriptsize(mm)}} & \parbox[t]{\linewidth}{\centering\textbf{$V_{\mathrm{oc}}$}\\[2pt]{\scriptsize(mV)}} & \parbox[t]{\linewidth}{\centering\textbf{BW}\\[2pt]{\scriptsize(MHz)}} & \parbox[t]{\linewidth}{\centering\textbf{SNR}\\[2pt]{\scriptsize(dB)}} & \parbox[t]{\linewidth}{\centering\textbf{$C_{\mathrm{match}}$}\\[2pt]{\scriptsize(Gbps)}} & \parbox[t]{\linewidth}{\centering\textbf{$C_{\mathrm{High\text{-}Z}}$}\\[2pt]{\scriptsize(Gbps)}} & \parbox[t]{\linewidth}{\centering\textbf{$L_{\mathrm{tis}}$}\\[2pt]{\scriptsize(dB)}} & \parbox[t]{\linewidth}{\centering\textbf{$L_{\mathrm{path}}$}\\[2pt]{\scriptsize(dB)}} & \parbox[t]{\linewidth}{\centering\textbf{$P_{\mathrm{tx}}$}\\[2pt]{\scriptsize(mW)}} \\
\midrule
NIC & 10 & 1104 & 0.4188 & 104.6 & 0.01456 & 0.01539 & 0.28 & 3.07 & 3.0$^{*}$ \\
 & 20 & 656.8 & 0.4188 & 100.1 & 0.01393 & 0.01477 & 0.95 & 6.92 & 3.0$^{*}$ \\
 & 30 & 361.9 & 0.4188 & 95.0 & 0.01321 & 0.01405 & 1.31 & 11.73 & 3.0$^{*}$ \\
\midrule
US & 10 & 537.2 & 0.0476 & 107.8 & 0.001705 & 0.0018 & 7.20 & 13.76 & 3.0$^{*}$ \\
 & 20 & 218.3 & 0.0476 & 100.0 & 0.001581 & 0.001677 & 7.53 & 21.25 & 3.0$^{*}$ \\
 & 30 & 164.8 & 0.0476 & 97.6 & 0.001543 & 0.001638 & 7.64 & 23.59 & 3.0$^{*}$ \\
\midrule
ME & 10 & 195.4 & 0.05298 & 98.6 & 0.001735 & 0.001841 & 0.01 & 33.41 & 3.0$^{*}$ \\
 & 20 & 165.9 & 0.05298 & 97.2 & 0.00171 & 0.001816 & 0.07 & 34.78 & 3.0$^{*}$ \\
 & 30 & 130.7 & 0.05298 & 95.1 & 0.001673 & 0.001779 & 0.10 & 36.82 & 3.0$^{*}$ \\
\midrule
BCC & 10 & 12.25 & 100 & 41.8 & 1.387 & 1.587 & 0.35 & 35.67 & 3.0$^{*}$ \\
 & 20 & 4.022 & 100 & 32.1 & 1.066 & 1.266 & 1.16 & 44.53 & 3.0$^{*}$ \\
 & 30 & 2.097 & 100 & 26.4 & 0.8784 & 1.078 & 1.63 & 49.72 & 3.0$^{*}$ \\
\midrule
UWB-700 & 10 & 60.8 & 700 & 47.2 & 10.98 & 12.38 & 9.03 & 4.48 & 0.4154$^{\#}$ \\
 & 20 & 30.4 & 700 & 41.2 & 9.582 & 10.98 & 15.32 & 10.50 & 1.7674$^{\#}$ \\
 & 30 & 10.34 & 700 & 31.8 & 7.405 & 8.805 & 22.65 & 14.03 & 2.49$^{+}$ \\
UWB-B4 & 10 & 91.46 & 1584 & 47.2 & 24.85 & 28.02 & 9.03 & 4.48 & 0.9401$^{\#}$ \\
 & 20 & 36.06 & 1584 & 39.1 & 20.6 & 23.76 & 15.32 & 10.50 & 2.49$^{+}$ \\
 & 30 & 10.34 & 1584 & 28.3 & 14.89 & 18.06 & 22.65 & 14.03 & 2.49$^{+}$ \\
\midrule
\multicolumn{10}{@{}p{14.5cm}@{}}{{\fontsize{6pt}{7.5pt}\selectfont $^{*}$~Max.\ power limit (thermal safety, 1\,$^\circ$C budget; applies to all non-UWB modalities and UWB when battery-limited).}}\\
\multicolumn{10}{@{}p{14.5cm}@{}}{{\fontsize{6pt}{7.5pt}\selectfont $^{\#}$~FCC~\S15.517 EIRP limit ($-41.3$\,dBm\,MHz$^{-1}$; 52\,$\mu$W at 700\,MHz, 117\,$\mu$W at B4 band at air interface; implant TX power scales as $P_{\mathrm{EIRP}}\times 10^{L_{\mathrm{tis}}/10}$).}}\\
\multicolumn{10}{@{}p{14.5cm}@{}}{{\fontsize{6pt}{7.5pt}\selectfont $^{+}$~SAR-1\,g limit, FCC~\S1.1310 (1.6\,W\,kg$^{-1}$ per 1\,g, grey matter).}}\\
\multicolumn{10}{@{}p{14.5cm}@{}}{{\fontsize{6pt}{7.5pt}\selectfont $^{\wedge}$~SAR-10\,g limit, ICNIRP~2020 (2.0\,W\,kg$^{-1}$ per 10\,g).}}\\
\bottomrule
\end{longtable}
}
}


==> tables/table4_geometry.tex <==
{
{\fontsize{8pt}{9pt}\selectfont
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.25}
\setlength{\baselineskip}{0pt}
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}

\begin{longtable}{@{}P{0.8cm}P{1.2cm}P{1.3cm}P{1.5cm}P{1.5cm}P{1.2cm}P{1.3cm}p{2.4cm}p{2.2cm}@{}}
\caption{\textbf{Geometry scaling from standard implant to $\sim$1\,mm$^3$ volume.} Standard geometries from Hosur et al., ISCAS~2025. US: rect.\ $6.4{\times}2.3{\times}1.4$\,mm$^3$ element, length-bar mode $f_r = v_\mathrm{bar}/(2L)$ ($v_\mathrm{bar}\!\approx\!3046$\,m\,s$^{-1}$), uniform scaling. ME: $f_r = v_L/(2L)$, $v_L$ from reference. UWB: $-7$\,dB efficiency; flat-die geometry ($12{\times}12{\times}0.05$\,mm$^3$) gives $k_t a\!\approx\!2.47\gg 1$ after scaling, Chu non-binding, BW FCC-limited at 700\,MHz.}
\label{tab:geom_scaling}\\
\toprule
\textbf{Mod.} & \parbox[t]{\linewidth}{\centering\textbf{$V_{\mathrm{oc,std}}$}\\[2pt]{\scriptsize(V)}} & \parbox[t]{\linewidth}{\centering\textbf{$V_{\mathrm{oc,1mm^3}}$}\\[2pt]{\scriptsize(V)}} & \parbox[t]{\linewidth}{\centering\textbf{$\Delta\mathrm{SNR}_{\mathrm{geom}}$}\\[2pt]{\scriptsize(dB)}} & \parbox[t]{\linewidth}{\centering\textbf{$\Delta\mathrm{SNR}_{\mathrm{path}}$}\\[2pt]{\scriptsize(dB)}} & \parbox[t]{\linewidth}{\centering\textbf{$\Delta\mathrm{BW}$}\\[2pt]{\scriptsize(dB)}} & \parbox[t]{\linewidth}{\centering\textbf{$C_{1\,\mathrm{mm}^3}$}\\[2pt]{\scriptsize(Gbps)}} & \textbf{Size change} & \textbf{BW / $f_r$ effect} \\
\midrule
NIC & 2.603 & 0.9076 & -9.2 & +0.0 & +0.0 & 0.01432 & $r_{\mathrm{Rx}}$: 1.05$\to$0.62\,mm & BW unchanged \\
\midrule
US & 13.66 & 1.287 & -17.5 & -3.0 & +4.4 & 0.004813 & $A$: 14.7$\to$1.96\,mm$^2$ & $f_r$: 238$\to$652\,kHz \\
\midrule
ME & 14 & 0.5612 & -27.4 & -0.5 & +4.6 & 0.005205 & Vol: 23.6$\to$1\,mm$^3$ & $f_r$: 279$\to$800\,kHz \\
\midrule
BCC & 0.1925 & 0.06128 & -9.9 & +0.0 & +0.0 & 1.852 & $r_{AB}$: 4$\to$1.27\,mm & Log-dist.\ path \\
\midrule
UWB & 0.005209 & 0.002327 & -7.0 & +0.0 & +0.0 & 4.404 & $a$: flat die, ${\approx}4.31$\,mm & FCC limited; Chu non-binding (flat die) \\
\bottomrule
\end{longtable}
}
}


==> tables/table_dims.tex <==
{
{\fontsize{8pt}{5pt}\selectfont
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.10}
\setlength{\baselineskip}{0pt}
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}

\begin{longtable}{@{}P{1.8cm}P{2.0cm}P{3.8cm}P{1.4cm}P{3.8cm}@{}}
\caption{\textbf{Active-element geometry of the five reference implants.} NIC, ME, and US dimensions from ~\cite{kiani_iscas25}; BCC ~\cite{ref144} (electrode separation $r_{AB} = 4.0$\,mm, body footprint $4.0 \times 2.5$\,mm); UWB reference die ~\cite{jung2025wireless} ($12 \times 12 \times 0.05$\,mm, subdural-contained neural recording SoC).}
\label{tab:dims}\\
\toprule
\textbf{Modality} & \textbf{Reference} & \textbf{Active-element dimensions} & \textbf{Vol.\ (mm$^3$)} & \textbf{Primary coupling dimension} \\
\midrule
NIC & \cite{kiani_iscas25} & Cylindrical coil, OD $2.1$\,mm, $h = 5.8$\,mm & $\approx 20$ & Coil OD $2.1$\,mm \\
\midrule
ME & \cite{kiani_iscas25} & $6.4 \times 2.3 \times 1.6$\,mm & $23.6$ & Bar length $6.4$\,mm \\
\midrule
US & \cite{kiani_iscas25} & $6.4 \times 2.3 \times 1.4$\,mm & $20.6$ & Face area $14.7$\,mm$^2$ \\
\midrule
BCC & \cite{ref144} & $4.0 \times 2.5$\,mm (footprint) & N/A & Electrode sep.\ $4.0$\,mm \\
\midrule
UWB\,(ref.\ die) & \cite{jung2025wireless} & $12 \times 12 \times 0.05$\,mm & $7.2$ & Die length $\approx 12$\,mm \\
\bottomrule
\end{longtable}
}
}


==> tables/table_geom_eqns.tex <==
{
{\fontsize{8pt}{10pt}\selectfont
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.10}
\setlength{\baselineskip}{0pt}
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}

\begin{longtable}{@{}P{0.9cm}p{5.5cm}p{4.0cm}p{3.8cm}@{}}
\caption{\textbf{Geometric and coupling models for the five uplink modalities.} $r_1$, $r_2$: transmit and receive coil radii; $A_{\mathrm{Rx}}$: transducer face area; $\alpha_{\mathrm{ac}}$: acoustic attenuation coefficient; $c_s \approx 1540$\,m\,s$^{-1}$: sound speed; $h$: piezo thickness; $\mathrm{Vol}$: ME stack volume; $H(d)$: BCC log-distance transfer function; $\alpha_{\mathrm{EM}}$: EM tissue absorption; $P_{\mathrm{tx}}$: UWB transmit power. }
\label{tab:geom_eqns}\\
\toprule
\textbf{Mod.} & \textbf{$V_{\mathrm{oc}}$ scaling with depth $d$} & \textbf{$f_r$ (resonant freq.)} & \textbf{$Q$} \\
\midrule
NIC & $V_{\mathrm{oc}} \propto r_1^2 r_2^2\,(r_1^2+d^2)^{-3/2}$ & External LC tank & $\approx 80$ (coil) \\
US & $V_{\mathrm{oc}} \propto A_{\mathrm{Rx}}\,e^{-\alpha_{\mathrm{ac}}d}/d$ & $f_r = c_s/(2h)$ (thickness) & $\approx 5$ (fluid-loaded) \\
ME & $V_{\mathrm{oc}} \propto \mathrm{Vol}\,(r_{\mathrm{Tx}}^2+d^2)^{-3/2}$ & $f_{\mathrm{bar}}$ (bar resonance) & $\approx 5.3$ (magneto-strictive) \\
BCC & $V_{\mathrm{oc}} \propto V_{\mathrm{tx}}\cdot 10^{H(d)/20}$, $H\!\propto\! d^{-2.4}$ & N/A\textsuperscript{\dag} (capacitive) & N/A\textsuperscript{\dag} \\
UWB & $V_{\mathrm{oc}} \propto \sqrt{P_{\mathrm{tx}}}\,e^{-\alpha_{\mathrm{EM}}d}/d$ & N/A\textsuperscript{\ddag} (spectral mask) & N/A\textsuperscript{\ddag} (wideband) \\
\midrule
\multicolumn{4}{@{}p{14.2cm}@{}}{{\fontsize{6pt}{8pt}\selectfont \textsuperscript{\dag}BCC operates in the EQS quasi-static regime (DC to 100\,MHz); the body channel is capacitive with no transducer resonance.}}\\
\multicolumn{4}{@{}p{14.2cm}@{}}{{\fontsize{6pt}{8pt}\selectfont \textsuperscript{\ddag}UWB bandwidth and power are governed by the FCC\,\S15.517 spectral EIRP mask ($-41.3$\,dBm\,MHz$^{-1}$); no resonant element is used.}}\\
\bottomrule
\end{longtable}
}
}


==> tables/table_uwb_depth.tex <==
{
{\fontsize{8pt}{5pt}\selectfont
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.80}
\setlength{\baselineskip}{0pt}
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}

\begin{longtable}{@{}P{1.5cm}P{0.7cm}P{1.0cm}P{1.0cm}P{1.0cm}P{1.2cm}P{1.9cm}P{1.4cm}P{1.0cm}P{1.0cm}P{1.1cm}@{}}
\caption{\textbf{UWB depth analysis with three-way power constraint.}\\$P_{\mathrm{tx}} = \min(P_{\mathrm{FCC\,comp}},\,P_{\mathrm{SAR\text{-}1g}},\,P_{\mathrm{SAR\text{-}10g}},\,P_{\mathrm{UL,max}})$. \\$P_{\mathrm{FCC\,comp}}$: TX power required to maintain surface EIRP at FCC~\S15.517 ($-41.3$\,dBm\,MHz$^{-1}$) after tissue loss. $\\P_{\mathrm{SAR\text{-}1g}} = 2.49$\,mW (FCC~\S1.1310: 1.6\,W\,kg$^{-1}$\,g$^{-1}$, grey matter). $\\P_{\mathrm{SAR\text{-}10g}} = 22.43$\,mW (ICNIRP~2020: 2.0\,W\,kg$^{-1}$, 10\,g). $\\P_{\mathrm{UL,max}} = 3$\,mW. FCC EIRP binding at $d \lesssim 20$\,mm; SAR-1\,g at $d \gtrsim 25$\,mm.}
\label{tab:uwb_depth}\\
\toprule
\textbf{BW} & \textbf{$d$ (mm)} & \textbf{$L_{\mathrm{tis}}$ (dB)} & \textbf{$L_{\mathrm{FSPL}}$ (dB)} & \textbf{$L_{\mathrm{tot}}$ (dB)} & \textbf{$P_{\mathrm{tx}}$ ($\mu$W)} & \textbf{Binding} & \textbf{$P_{\mathrm{rx}}$ ($\mu$W)} & \textbf{$V_{\mathrm{oc}}$ (mV)} & \textbf{SNR (dB)} & \textbf{$C$} \\
\midrule
700 MHz & 10 & 9.03 & 4.48 & 13.52 & 415.44 & FCC\text{-}EIRP & 18.4842 & 60.80 & 47.2 & 10.98\,Gb\,s$^{-1}$ \\
 & 20 & 15.32 & 10.50 & 25.83 & 1767.43 & FCC\text{-}EIRP & 4.6211 & 30.40 & 41.2 & 9.58\,Gb\,s$^{-1}$ \\
 & 30 & 22.65 & 14.03 & 36.67 & 2486.61 & SAR\text{-}1g & 0.5349 & 10.34 & 31.8 & 7.41\,Gb\,s$^{-1}$ \\
\midrule
1584 MHz & 10 & 9.03 & 4.48 & 13.52 & 940.08 & FCC\text{-}EIRP & 41.8271 & 91.46 & 47.2 & 24.85\,Gb\,s$^{-1}$ \\
 & 20 & 15.32 & 10.50 & 25.83 & 2486.61 & SAR\text{-}1g & 6.5014 & 36.06 & 39.1 & 20.60\,Gb\,s$^{-1}$ \\
 & 30 & 22.65 & 14.03 & 36.67 & 2486.61 & SAR\text{-}1g & 0.5349 & 10.34 & 28.3 & 14.89\,Gb\,s$^{-1}$ \\
\bottomrule
\end{longtable}
}
}

